Generating Configurable Hardware from Parallel Patterns

In recent years the computing landscape has seen an in- creasing shift towards specialized accelerators. Field pro- grammable gate arrays (FPGAs) are particularly promising as they offer significant performance and energy improvements compared to CPUs for a wide class of applications and are far more flexible than fixed-function ASICs. However, FPGAs are difficult to program. Traditional programming models for reconfigurable logic use low-level hardware description languages like Verilog and VHDL, which have none of the pro- ductivity features of modern software development languages but produce very efficient designs, and low-level software lan- guages like C and OpenCL coupled with high-level synthesis (HLS) tools that typically produce designs that are far less efficient. Functional languages with parallel patterns are a better fit for hardware generation because they both provide high-level abstractions to programmers with little experience in hard- ware design and avoid many of the problems faced when gen- erating hardware from imperative languages. In this paper, we identify two optimizations that are important when using par- allel patterns to generate hardware: tiling and metapipelining. We present a general representation of tiled parallel patterns, and provide rules for automatically tiling patterns and gen- erating metapipelines. We demonstrate experimentally that these optimizations result in speedups up to 40x on a set of benchmarks from the data analytics domain.

==> figs/speedupbars.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9360.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,1880){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2047){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2213){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,2380){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,2546){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(682,2713){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,2879){\makebox(0,0)[r]{\strut{}$12$}}%
      \put(2172,1660){\makebox(0,0){\strut{}outerprod}}%
      \put(3530,1660){\makebox(0,0){\strut{}sumrows}}%
      \put(4889,1660){\makebox(0,0){\strut{}matmult}}%
      \put(6247,1660){\makebox(0,0){\strut{}tpchq1}}%
      \put(7605,1660){\makebox(0,0){\strut{}tpchq6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2379){\rotatebox{-270}{\makebox(0,0){\strut{}speedup}}}%
      \csname LTb\endcsname%
      \put(1765,2563){\makebox(0,0){\strut{}7}}%
      \put(3123,2563){\makebox(0,0){\strut{}7}}%
      \put(4481,2563){\makebox(0,0){\strut{}7}}%
      \put(5839,2563){\makebox(0,0){\strut{}7}}%
      \put(7197,2563){\makebox(0,0){\strut{}7}}%
      \csname LTb\endcsname%
      \put(2036,2729){\makebox(0,0){\strut{}9}}%
      \put(3395,2729){\makebox(0,0){\strut{}9}}%
      \put(4753,2729){\makebox(0,0){\strut{}9}}%
      \put(6111,2729){\makebox(0,0){\strut{}9}}%
      \put(7469,2729){\makebox(0,0){\strut{}9}}%
      \csname LTb\endcsname%
      \put(2308,2063){\makebox(0,0){\strut{}1}}%
      \put(3666,2063){\makebox(0,0){\strut{}1}}%
      \put(5024,2063){\makebox(0,0){\strut{}1}}%
      \put(6382,2063){\makebox(0,0){\strut{}1}}%
      \put(7741,2063){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%
      \put(2580,2146){\makebox(0,0){\strut{}2}}%
      \put(3938,2146){\makebox(0,0){\strut{}2}}%
      \put(5296,2146){\makebox(0,0){\strut{}2}}%
      \put(6654,2146){\makebox(0,0){\strut{}2}}%
      \put(8012,2146){\makebox(0,0){\strut{}2}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,440){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,607){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,773){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,940){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,1107){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(682,1273){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,1440){\makebox(0,0)[r]{\strut{}$12$}}%
      \put(2172,220){\makebox(0,0){\strut{}sobel}}%
      \put(3530,220){\makebox(0,0){\strut{}logreg}}%
      \put(4889,220){\makebox(0,0){\strut{}gda}}%
      \put(6247,220){\makebox(0,0){\strut{}kmeans}}%
      \put(7605,220){\makebox(0,0){\strut{}knn}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,940){\rotatebox{-270}{\makebox(0,0){\strut{}speedup}}}%
      \csname LTb\endcsname%
      \put(1765,1123){\makebox(0,0){\strut{}7}}%
      \put(3123,1123){\makebox(0,0){\strut{}7}}%
      \put(4481,1123){\makebox(0,0){\strut{}7}}%
      \put(5839,1123){\makebox(0,0){\strut{}7}}%
      \put(7197,1123){\makebox(0,0){\strut{}7}}%
      \csname LTb\endcsname%
      \put(2036,1290){\makebox(0,0){\strut{}9}}%
      \put(3395,1290){\makebox(0,0){\strut{}9}}%
      \put(4753,1290){\makebox(0,0){\strut{}9}}%
      \put(6111,1290){\makebox(0,0){\strut{}9}}%
      \put(7469,1290){\makebox(0,0){\strut{}9}}%
      \csname LTb\endcsname%
      \put(2308,623){\makebox(0,0){\strut{}1}}%
      \put(3666,623){\makebox(0,0){\strut{}1}}%
      \put(5024,623){\makebox(0,0){\strut{}1}}%
      \put(6382,623){\makebox(0,0){\strut{}1}}%
      \put(7741,623){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%
      \put(2580,707){\makebox(0,0){\strut{}2}}%
      \put(3938,707){\makebox(0,0){\strut{}2}}%
      \put(5296,707){\makebox(0,0){\strut{}2}}%
      \put(6654,707){\makebox(0,0){\strut{}2}}%
      \put(8012,707){\makebox(0,0){\strut{}2}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/speedupbars}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> text/systemOverview.tex <==
\section{System Overview}
Figure \ref{} describes the steps in our approach for one of our benchmarks.

%\input{text/blockDiagram}
%\input{text/blocking}
%\input{text/hardwareGeneration}

